Monocular Marker-free Patient-to-Image Intraoperative Registration for Cochlear Implant Surgery

This paper presents a novel method for monocular patient-to-image intraoperative registration, specifically designed to operate without any external hardware tracking equipment or fiducial point markers. Leveraging a synthetic microscopy surgical scene dataset with a wide range of transformations, our approach directly maps preoperative CT scans to 2D intraoperative surgical frames through a lightweight neural network for real-time cochlear implant surgery guidance via a zero-shot learning approach. Unlike traditional methods, our framework seamlessly integrates with monocular surgical microscopes, making it highly practical for clinical use without additional hardware dependencies and requirements. Our method estimates camera poses, which include a rotation matrix and a translation vector, by learning from the synthetic dataset, enabling accurate and efficient intraoperative registration. The proposed framework was evaluated on nine clinical cases using a patient-specific and cross-patient validation strategy. Our results suggest that our approach achieves clinically relevant accuracy in predicting 6D camera poses for registering 3D preoperative CT scans to 2D surgical scenes with an angular error within 10 degrees in most cases, while also addressing limitations of traditional methods, such as reliance on external tracking systems or fiducial markers.

==> trashcan.tex <==
In our proposed method, we have the postmastoidectomy surfaces $\mathcal{V} = (\mathbf{v}, \mathbf{f})$ extracted from the preoperative CT scans, the synthetic 2D monocular surgical microscope images $\mathcal{I} \in \mathbb{R}^{H \times W}$ and their corresponding camera extrinsic matrix $\mathcal{P} = [\mathcal{R}|t]$. We define a set of 3D vertices $\mathbf{v} = \{v_i \in \mathbb{R}^{N\times3}\} \subset \mathcal{V} $ and a set of triangle faces $\mathbf{f} = \{f_i \in \mathbb{Z}^{N'\times3}\} \subset \mathcal{V}$, where $N$ and $N'$ represents the number of vertices and faces, respectively.



In our proposed method, we have the postmastoidectomy surfaces extracted from the preoperative CT scans, the synthetic 2D monocular surgical microscope images $\mathcal{I} \in \mathbb{R}^{H \times W}$ and their corresponding camera extrinsic matrix $\mathcal{P} = [\mathcal{R}|t]$. $H$ and $W$ denote the height and the width of $\mathcal{I}$, $\mathcal{R} \in SO(3)$ represents the rotation matrix, and $t \in \mathbb{R}^3$ is the translation vector.


The rotational error $d_{rot}$ between vector $\mathcal{R}$ and $\mathcal{R}'$ is defined as $d_{rot} = \norm{\mathcal{R}' - \mathcal{R}}_2$, while the translational error $d_{t}$ between $t$ and $t'$ is given by $d_{t} = \abs{t' - t}$. 

Note that in our experiment settings, all $\mathcal{R}$ are derived from an initial pose $\mathcal{R}_0$ within $\pm20^{\circ}$ angular distance. 

``Synth$\rightarrow$Synth'' denotes models trained and tested exclusively on the synthetic post-mastoidectomy surface dataset, while

% To ensure a fair comparison with the method proposed in \cite{10.1117/12.3008830}, we evaluated both approaches on real surgical scenes by predicting their corresponding camera poses. Our proposed method achieves a N\% improvement in BLAH metric, illustrating how using the entire observable CT instead of small and occluded landmarks for patient-to-image intraoperative registration is more robust in terms of the depth estimation. Moreover, the use of synthetic dataset to supplement the training of the model address data scarcity and clearly improves the model's BLAH metric performance by obtaining a M\% enhancement.


% , is shown in Equation~\ref{eq:d_rot}
% \begin{equation}
%     D_{rot} = \arccos\left(\frac{\mathrm{Tr}(\mathcal{R}^T\mathcal{R}') - 1}{2}\right)
% \label{eq:d_rot}
% \end{equation}

within the critical 10-degree range

$E_{t}$ was predominantly contributed by the z-translation error in most cases, indicating that most of the translational offset occurred along the depth axis. 

To optimize the objective function, we develop a pose regression model $f_\theta$ based on the state-of-the-art Kolmogorov-Arnold Networks (KAN) \cite{liu2024kankolmogorovarnoldnetworks,drokin2024kolmogorovarnoldconvolutionsdesignprinciples}, specifically designed for the 3D-to-2D intraoperative registration task. The model shown in Figure~\ref{fig:framework} is trained exclusively on a synthetic surgical dataset with pre-defined camera poses $\mathcal{P}$.



% \begin{figure}[htbp]
%   \centering
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%   \end{minipage}
%   % new line
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%   \end{minipage}
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%   \end{minipage}
%   % new line
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%       \footnotesize{Case 1}
%   \end{minipage}
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%       \footnotesize{Case 2}
%   \end{minipage}
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%       \footnotesize{Case 3}
%   \end{minipage}
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%       \footnotesize{Case 4}
%   \end{minipage}
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%       \footnotesize{Case 5}
%   \end{minipage}
%   \begin{minipage}[b]{0.15\textwidth}
%       \centering
%       \includegraphics[width=\textwidth]{figures/frame_168.png}
%       \footnotesize{Case 6}
%   \end{minipage}
%   \caption{\textbf{Qualitative Evaluation}. We present both the patient-specific and cross-patient results on randomly selected surgical scenes from 3 different patients.}
%   \label{fig:qualitative_results}
% \end{figure}




\begin{figure}[ht]
    %--- First block of two images
    \begin{minipage}[t]{0.45\textwidth}
        \begin{minipage}[c]{0.05\textwidth}
            \centering
            \rotatebox{90}{Original}
        \end{minipage}
        \begin{minipage}{0.45\textwidth}
            \includegraphics[width=\textwidth]{figures/frame_168.png}
        \end{minipage}
        % \begin{minipage}{0.3\textwidth}
        %     \includegraphics[width=\textwidth]{figures/frame_168.png}
        % \end{minipage}
        \begin{minipage}{0.45\textwidth}
            \includegraphics[width=\textwidth]{figures/frame_168.png}
        \end{minipage}
    \end{minipage}
    \hspace{2em}
    %--- Second block of two images
    \begin{minipage}[t]{0.45\textwidth}
        \begin{minipage}[c]{0.05\textwidth}
            \centering
            \rotatebox{90}{Original}
        \end{minipage}
         \begin{minipage}{0.45\textwidth}
            \includegraphics[width=\textwidth]{figures/frame_168.png}
        \end{minipage}
        % \begin{minipage}{0.3\textwidth}
        %     \includegraphics[width=\textwidth]{figures/frame_168.png}
        % \end{minipage}
        \begin{minipage}{0.45\textwidth}
            \includegraphics[width=\textwidth]{figures/frame_168.png}
        \end{minipage}
    \end{minipage}

    %--- First block of two images
    \begin{minipage}[t]{0.45\textwidth}
        \begin{minipage}[c]{0.05\textwidth}
            \centering
            \rotatebox{90}{Pose $\mathcal{P}'$}
        \end{minipage}
        \begin{minipage}{0.45\textwidth}
            \includegraphics[width=\textwidth]{figures/frame_168.png}
        \end{minipage}
        % \begin{minipage}{0.3\textwidth}
        %     \includegraphics[width=\textwidth]{figures/frame_168.png}
        % \end{minipage}
        \begin{minipage}{0.45\textwidth}
            \includegraphics[width=\textwidth]{figures/frame_168.png}
        \end{minipage}
    \end{minipage}
    \hspace{2em}
    %--- Second block of two images
    \begin{minipage}[t]{0.45\textwidth}
        \begin{minipage}[c]{0.05\textwidth}
            \centering
            \rotatebox{90}{Pose $\mathcal{P}'$}
        \end{minipage}
        \begin{minipage}{0.45\textwidth}
            \includegraphics[width=\textwidth]{figures/frame_168.png}
        \end{minipage}
        % \begin{minipage}{0.3\textwidth}
        %     \includegraphics[width=\textwidth]{figures/frame_168.png}
        % \end{minipage}
        \begin{minipage}{0.45\textwidth}
            \includegraphics[width=\textwidth]{figures/frame_168.png}
        \end{minipage}
    \end{minipage}

    %--- First block of two images
    \begin{minipage}[t]{0.45\textwidth}
        \begin{minipage}[c]{0.05\textwidth}
            \centering
            \rotatebox{90}{Error}
        \end{minipage}
        \begin{minipage}{0.45\textwidth}
            \includegraphics[width=\textwidth]{figures/frame_168.png}
        \end{minipage}
        % \begin{minipage}{0.3\textwidth}
        %     \includegraphics[width=\textwidth]{figures/frame_168.png}
        % \end{minipage}
        \begin{minipage}{0.45\textwidth}
            \includegraphics[width=\textwidth]{figures/frame_168.png}
        \end{minipage}
    \end{minipage}
    \hspace{2em}
    %--- Second block of two images
    \begin{minipage}[t]{0.45\textwidth}
        \begin{minipage}[c]{0.05\textwidth}
            \centering
            \rotatebox{90}{Error}
        \end{minipage}
        \begin{minipage}{0.45\textwidth}
            \includegraphics[width=\textwidth]{figures/frame_168.png}
        \end{minipage}
        % \begin{minipage}{0.3\textwidth}
        %     \includegraphics[width=\textwidth]{figures/frame_168.png}
        % \end{minipage}
        \begin{minipage}{0.45\textwidth}
            \includegraphics[width=\textwidth]{figures/frame_168.png}
        \end{minipage}
    \end{minipage}

    %--- First block of two images
    \begin{minipage}[t]{0.45\textwidth}
        \begin{minipage}[c]{0.05\textwidth}
            \centering
            \rotatebox{90}{Overlay}
        \end{minipage}
        \begin{minipage}{0.45\textwidth}
            \includegraphics[width=\textwidth]{figures/frame_168.png}
            \centering
            \footnotesize{Sample 1}
        \end{minipage}
        % \begin{minipage}{0.3\textwidth}
        %     \includegraphics[width=\textwidth]{figures/frame_168.png}
        %     \centering
        %     \footnotesize{Sample 2}
        % \end{minipage}
        \begin{minipage}{0.45\textwidth}
            \includegraphics[width=\textwidth]{figures/frame_168.png}
            \centering
            \footnotesize{Sample 2}
        \end{minipage}
        
        \centering
        \vspace{1em}Patient-Specific
    \end{minipage}
    \hspace{2em}
    %--- Second block of two images
    \begin{minipage}[t]{0.45\textwidth}
        \begin{minipage}[c]{0.05\textwidth}
            \centering
            \rotatebox{90}{Overlay}
        \end{minipage}
        \begin{minipage}{0.45\textwidth}
            \includegraphics[width=\textwidth]{figures/frame_168.png}
            \centering
            \footnotesize{Sample 1}
        \end{minipage}
        % \begin{minipage}{0.3\textwidth}
        %     \includegraphics[width=\textwidth]{figures/frame_168.png}
        %     \centering
        %     \footnotesize{Sample 2}
        % \end{minipage}
        \begin{minipage}{0.45\textwidth}
            \includegraphics[width=\textwidth]{figures/frame_168.png}
            \centering
            \footnotesize{Sample 2}
        \end{minipage}
       
        \centering
        \vspace{1em}Cross-Patient
    \end{minipage}
    \caption{\textbf{Qualitative Evaluation}. We present both the patient-specific and cross-patient results on randomly selected surgical scenes from 3 different patients.}
  \label{fig:qualitative_results}
\end{figure}


% CNN based network table
\begin{table}[]
    \centering
    \begin{tabular}{c|c| *{8}{>{\centering\arraybackslash}p{\rowSize{}}|} *{1}{>{\centering\arraybackslash}p{\rowSize{}}} }
        \toprule
        Metric & Experiments & C1 & C2 & C3 & C4 & C5 & C6 & C7 & C8 & C9 \\
        \midrule
        \rowcolor{\rowColorOne}
        % & Synth$\rightarrow$Synth & 13.59 & 20.19 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
        % \cmidrule{2-11}
        \rowcolor{\rowColorTwo}
        ADD & Patient-specific & 176.5 & 92.98 & 82.93 & 99.44 & 135.7 & 134.9 & 102.5 & 125.5 & 142.5 \\
        \rowcolor{\rowColorThree}
        (mm) & Cross-patient & 212.6 & 140.9 & 85.71 & 117.8 & 133.0 & 81.58 & 75.69 & 54.83 & 82.75 \\
        \midrule
        % \rowcolor{\rowColorOne}
        % & Synth$\rightarrow$Synth & 5.51 & 4.80 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
        % \cmidrule{2-11}
        \rowcolor{\rowColorTwo}
        $E_{rot}$ & Patient-specific & 2.74 & 2.39 & 1.47 & 4.15 & 3.08 & 2.59 & 1.49 & 5.32 & 2.26 \\
        \rowcolor{\rowColorThree}
        ($n^{\circ}$) & Cross-patient & 9.08 & 8.73 & 12.89 & 5.00 & 6.29 & 5.37 & 6.64 & 6.83 & 6.22 \\
        \midrule
        % \rowcolor{\rowColorOne}
        % & Synth$\rightarrow$Synth & 16.16 & 21.20 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\
        % \cmidrule{2-11}
        \rowcolor{\rowColorTwo}
        $E_{t}$ & Patient-specific & 178.3 & 92.09 & 85.35 & 96.31 & 134.0 & 135.0 & 102.0 & 114.5 & 141.4 \\
        \rowcolor{\rowColorThree}
        (mm) & Cross-patient & 209.2 & 149.1 & 91.11 & 119.9 & 134.4 & 80.52 & 77.41 & 41.28 & 76.33 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Quantitative Evaluation}. This table presents both patient-specific and cross-patient assessments. C1 represents Case 1.}
    \label{tab:quantitative_evaluation}
\end{table}

For the \textit{patient-specific}, the average ADD, $E_{rot}$, and $E_{t}$ are 121.44 mm, 2.83$^\circ$, and 119.88 mm, respectively. For the \textit{cross-patient}, they are 109.43 mm, 7.45$^\circ$, and 108.81 mm across all cases. 

To optimize the objective function, we develop a pose regression model $f_\theta$ based on the state-of-the-art Kolmogorov-Arnold Networks (KAN) \cite{liu2024kankolmogorovarnoldnetworks,drokin2024kolmogorovarnoldconvolutionsdesignprinciples}, specifically designed for the 3D-to-2D intraoperative registration task. The model shown in Figure~\ref{fig:framework} is trained exclusively on a synthetic surgical dataset with pre-defined camera poses $\mathcal{P}$.

% . The cross-patient results suggest the method's potential to generalize to new patients, showing scalability while addressing real data scarcity challenges through the use of synthetic datasets.
